Verified Rust Monitors for Lola Specifications

The safety of cyber-physical systems rests on the correctness of their monitoring mechanisms. This is problematic if the specification of the monitor is implemented manually or interpreted by unreliable software. We present a verifying compiler that translates specifications given in the stream-based monitoring language Lola to implementations in Rust. The generated code contains verification annotations that enable the Viper toolkit to automatically prove functional correctness, absence of memory faults, and guaranteed termination. The compiler parallelizes the evaluation of different streams in the monitor based on a dependency analysis of the specification. We present encouraging experimental results obtained with monitor specifications found in the literature. For every specification, our approach was able to either produce a correctness proof or to uncover errors in the specification.

==> figures/codestructure.tex <==
\begin{lstlisting}[style=ColoredRust]
struct Memory { ... } $\tikzmark{preludeBegin}$
impl Memory { $\dots$ }
fn eval_$s_{1,1}$(mem: &Memory) -> $T_{s_{1,1}}$ { ... }
...
fn eval_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$(mem: &Memory) -> $T_{s_{1,1}}$ { ... }
fn eval_pre_1_$s_{1,1}$(&memory) -> $T_{s_{1,1}}$ { ... }
    ...
fn eval_pre_1_$s_{1,\lambda_1}$(&memory) -> $T_{s_{1,\lambda_1}}$ { ... }
    ...
fn eval_pre_$s_{\lambda^\ast,1}$(&memory) -> $T_{s_{\lambda^\ast,1}}$ { ... }
    ...
fn eval_pre_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$(&memory) -> $T_{s_{\lambda^\ast,\lambda_{\lambda^\ast}}}$ { ... }
fn get_input() -> Option<($T_{s_1}, \dots, T_{s_\ell}$)> {
  [[ Communicate with system ]]
}
fn emit(output: &($T_{s_1}, \dots, T_{s_n}$)) {
  [[ Communicate with system ]]
}
fn main() {
  let mut memory = Memory::new(); $\tikzmark{preludeEnd}$
  if let Some(input1) = get_input() {$\tikzmark{prefixBegin}$
    mem.add_input(&input1)
    let val_$s_{1,1}$ = eval_pre_1_$s_{1,1}$(&memory);
    ...
    let val_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$ = eval_pre_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$(&memory);
    memory.write_layer_$\lambda^\ast$(val_$s_{\lambda^\ast,1}$, ..., val_$s_{\lambda^\ast, \lambda_{\lambda^\ast}}$);$\tikzmark{longest}$
    if val_$s_{t_1}$ == true { emit($m_{t_1}$) }
    ...
    if val_$s_{t_{t^\ast}}$ == true { emit($m_{t_1}$) }
  } else { $\dots$ }
  [[ Repeat $\color[rgb]{0.6, 0.4, 0.08}\postlen$ times. ]] $\tikzmark{prefixEnd}$

  while let Some(input) = get_input() { $\tikzmark{loopBegin}$
    mem.add_input(&input1)
    let val_$s_{1,1}$ = eval_$s_{1,1}$(&memory);
    ...
    let val_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$ = eval_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$
    memory.write_layer_$\lambda^\ast$(val_$s_{\lambda^\ast,1}$, ..., val_$s_{\lambda^\ast, \lambda_{\lambda^\ast}}$);
    if val_$s_{t_1}$ == true { emit($m_{t_1}$) }
    [[ Repeat for each trigger ]]
  } $\tikzmark{loopEnd}$

  let val_$s_{1,1}$ = eval_post_1_$s_{1,1}$(&memory)$\tikzmark{postfixBegin}$;
  ...
  let val_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$ = eval_$s_{\lambda^\ast,\lambda_{\lambda^\ast}}$
  memory.write_layer_$\lambda^\ast$(val_$s_{\lambda^\ast,1}$, ..., val_$s_{\lambda^\ast, \lambda_{\lambda^\ast}}$)
  if val_$s_{t_1}$ == true { emit($m_{t_1}$) }
  [[ Repeat for each trigger ]]
  [[ Repeat $\color[rgb]{0.6, 0.4, 0.08}\postlen$ times. ]]$\tikzmark{postfixEnd}$
}
\end{lstlisting}
  \AddNote{preludeBegin}{preludeEnd}{longest}{Prelude}
  \AddNote{prefixBegin}{prefixEnd}{longest}{Prefix}
  \AddNote{loopBegin}{loopEnd}{longest}{Monitor\\Loop}
  \AddNote{postfixBegin}{postfixEnd}{longest}{Postfix}


==> motivation.tex <==
\section{Motivation (1.5p)}\label{sec:motivation}

Drones are a common target for runtime verification. 
For instance, it is easy to detect whether a drone flies below a given minimum altitude too long and to raise an alarm if needed. 
This can be specified in \lola as follows:
%
\begin{lstlisting}[style=LolaDefault]
input altitude: Int
output tooLow: Bool := altitude[1,0] < 200 && altitude < 200 && altitude[-1,0] < 200
output tooHigh: Bool := altitude[1,0] > 600 && altitude > 600 && altitude[-1,0] > 600
trigger tooLow "Flying below minimum altitude"
trigger tooHigh "Flying above maximum altitude"
\end{lstlisting}

The input stream \texttt{altitude} contains sensor information of the drone. 
The output stream \texttt{tooLow} checks whether the altitude is lower than the given minimum altitude of \texttt{200} in the current, the last (\texttt{altitude[-1,0]}), and the next (\texttt{altitude[1,0]}) step.
If this is the case, a trigger is raised.
Analogously, the output stream \texttt{tooSlow} checks whether the altitude is lower than the given maximum altitude in the last, current, and next step. A trigger is raised in this case.

To verify the correctness of the monitor, we translate the specification into rust code containing verification conditions. 
Since the above \lola specification contains future offsets, in particular \texttt{altitude[1,0]}, the translation has to delay the computations of \texttt{tooLow} and \texttt{tooHigh} by one step.
In order to derive all computation delays induced by a \lola specification, we analyze its dependency graph. 
The one for the above specification is shown in Figure~\ref{fig:dep_graph_motivation}.
%
\begin{figure}[t]
	\begin{center}
	\begin{tikzpicture}[->,shorten >=2pt,auto,offset/.style={fill=white, anchor=center, pos=0.5, inner sep=3pt}]

			\node[state,ellipse]		(alt)		at (4,-0.75)			{altitude};
			\node[state,ellipse]		(tl)			at (0,0)			{tooLow};
			\node[state,ellipse]		(th)			at (0,-1.5)		{tooHigh};
			\node[state,ellipse]		(tr1)		at (-3,0)	{trigger};
			\node[state,ellipse]		(tr2)		at (-3,-1.5)	{trigger};
			
			\path	(tl)		edge							node[offset]		{$-1, 0, 1$}	(alt)
					(th)		edge							node[offset]		{$-1, 0, 1$}	(alt)
					(tr1)	edge							node	[offset]		{$0$}	(tl)
					(tr2)	edge							node[offset]		{$0$}	(th);
		\end{tikzpicture}
	\end{center}
	\caption{TODO}\label{fig:dep_graph_motivation}
\end{figure} 
%
The nodes denote the streams, edges denote stream accesses and, their weight corresponds to the offset of the access.
Hence, edges with positive weights imply computation delays.
In particular, the above specification introduces two computation delays, namely the one of \texttt{tooLow} and \texttt{tooHigh}.

While the output streams \texttt{tooLow} and \texttt{tooHigh} both depend on the input stream \texttt{altitude}, they do not depend on each other. 
Thus, since stream accesses are read-only, their evaluation is interleaving invariant, i.e.\ an arbitrary scheduler cannot change the result of the evaluations of \texttt{tooLow} and \texttt{tooHigh} or introduce data races.
In particular, \texttt{tooLow} and \texttt{tooHigh} can be evaluation concurrently.\todo{more details when definitions and proofs are final}

\todo[inline]{Rust Code with Verification Conditions}
